Back to the Drawing Board: A Critical Evaluation of Poisoning Attacks on Production Federated Learning

While recent works have indicated that federated learning (FL) may be vulnerable to poisoning attacks by compromised clients, their real impact on production FL systems is not fully understood. In this work, we aim to develop a comprehensive systemization for poisoning attacks on FL by enumerating all possible threat models, variations of poisoning, and adversary capabilities. We specifically put our focus on untargeted poisoning attacks, as we argue that they are significantly relevant to production FL deployments. We present a critical analysis of untargeted poisoning attacks under practical, production FL environments by carefully characterizing the set of realistic threat models and adversarial capabilities. Our findings are rather surprising: contrary to the established belief, we show that FL is highly robust in practice even when using simple, low-cost defenses. We go even further and propose novel, state-of-the-art data and model poisoning attacks, and show via an extensive set of experiments across three benchmark datasets how (in)effective poisoning attacks are in the presence of simple defense mechanisms. We aim to correct previous misconceptions and offer concrete guidelines to conduct more accurate (and more realistic) research on this topic.

==> experimental_setup.tex <==
% !TEX root = main.tex

\subsection{Experimental setup} \label{exp_setup}

\subsubsection{Datasets and Model Architectures}

\paragraphb{FEMNIST~\cite{caldas2018leaf,cohen2017emnist}} is a character recognition classification task with 3,400 clients, 62 classes (52 for upper and lower case letters and 10 for digits), and 671,585  grayscale images. 
Each client has data of her own handwritten digits or letters. Considering the huge number of clients in real-world cross-device FL (up to $10^{10}$), we further divide each of the clients' data in $p\in\{2,5,10\}$ non-iid parts using Dirichlet distribution~\cite{minka2000estimating} with $\alpha=1$. Increasing the Dirichlet distribution parameter, $\alpha$, generates more iid datasets. Unless specified otherwise, we set $p=10$, i.e., the total number of clients is 34,000. We use LeNet~\cite{lecun1998gradient} architecture.
% FEMNIST is a non-iid, class-imbalanced dataset commonly encountered in cross-device FL settings~\cite{kairouz2019advances}, while the previous datasets are more common in cross-silo FL settings.


\paragraphb{CIFAR10~\cite{krizhevsky2009learning}} is a 10-class classification task with 60,000 RGB images (50,000 for training and 10,000 for testing), each of size 32 $\times$ 32.
% `Class-balanced' datasets have the same number of samples per class, e.g., each class of CIFAR10 has 6,000 images.
% We use 5000 clients each with 1,000 samples and use validation and test data of sizes 5,000 each. 
Unless specified otherwise, we consider 1,000 total FL clients and divide the 50,000 training data using Dirichlet distribution~\cite{minka2000estimating} with $\alpha=1$. We use VGG9~\cite{simonyan2014very} architecture.

\paragraphb{Purchase~\cite{purchase}} is a   classification task with 100 classes and 197,324 binary feature vectors each of length 600. We use 187,324 of total data for training and divide it among 5,000 clients using Dirichlet distribution with $\alpha=1$. We use validation and test data of sizes 5,000 each. We use a fully connected network with layer sizes \{600, 1024, 100\}. Due to space restriction, we defer the details of the parameters of FL training and various attacks to Section~\ref{appdx:setup}.

% \vspace*{-.75em}
\subsubsection{Measurement Metric}\label{metric}
%
$A_\theta$ denotes the maximum accuracy achieved by the global model over all  FL training rounds, without any attack. $A^*_\theta$ for an attack denotes the maximum accuracy of the model under the given attack. We define \emph{attack impact}, $I_\theta$, as \emph{the reduction in the accuracy of the global model due to the attack}, hence for a given attack,  $I_\theta = A_\theta - A^*_\theta$.



==> fl_poisoning_dimensions.tex <==
% !TEX root = main.tex


\begin{table*}
% \vspace{-2em}
\centering
\fontsize{9}{10}\selectfont{}
\setlength{\extrarowheight}{0.05cm}
\caption{A valid combination of various dimensions discussed below constitutes a threat model for poisoning attack on FL.}
\label{table:poisoning_dimensions}

\begin{tabular}{ |c|p{2cm}|p{12cm}| } 
\hline

\textbf{Dimension} & \textbf{Values} & \textbf{Description} \\ \hline

\multirow{2}{2cm}{Adversary's goal ($\mathcal{G}$)} & Targeted (\texttt{T}) & Adversary aims to misclassify the samples with specific properties of her choice. \\ \cline{2-3}

& Untargeted (\texttt{UT})& Adversary aims to misclassify any sample input to the global model. \\ \hline
\hline


\multirow{4}{2cm}{Adversary's capability ($\mathcal{C}$)} & \multirow{2}{2cm}{Model poison (\texttt{MP})} & Adversary can directly manipulate the proprietary client updates. For this, adversary should completely break in to a client device, which also allows access data and model parameters.  \\
& & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-capabilities_model.pdf}}\\ \cline{2-3}

& \multirow{2}{2cm}{Data poison (\texttt{DP})} & Adversary can only manipulate the data on client device which the client uses to compute its updates. Adversary does not break in to client devices, hence cannot access model parameters or manipulate updates.\\ 
& & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-capabilities_data.pdf}} \\ \hline \hline







\multirow{6}{2cm}{Adversary's knowledge of global model ($\mathcal{K}$)} & \multirow{2}{2cm}{Nobox (\texttt{Nb})} & Adversary can neither access the global model parameters or its predictions nor can directly manipulate the client updates. \\
& & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-nobox-hcrop.pdf}} \\ \cline{2-3}

% & \multirow{2}{2cm}{Blackbox} & Adversary can only access the output predictions of the global model, but neither can access its parameters nor can manipulate the client updates.\\
% & & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-blackbox-hcrop.pdf}}\\ \cline{2-3}

% & \multirow{2}{2cm}{Graybox} & Adversary can access the global model parameters, and therefore, its predictions, but cannot manipulate the client updates. \\
% & & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-grayboxh.pdf}}\\ \cline{2-3}

& \multirow{2}{2cm}{Whitebox (\texttt{Wb})} & Adversary can access the global model parameters, its predictions, and can also manipulate the client updates.\\ 
& & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-whiteboxh.pdf}}\\ \hline
\hline




\multirow{4}{2cm}{Attack mode ($\mathcal{M}$)} & \multirow{2}{2cm}{Offline (\texttt{Off})} & Adversary can corrupt the compromised clients only once at the beginning of FL training. Such corruption may have very negligible impact on the updates that malicious clients share in later FL rounds.\\
&  & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-offline.pdf}} \\ \cline{2-3}

& \multirow{2}{2cm}{Online (\texttt{On})} & Due to the nature of FL, adversary can repeatedly and adaptively corrupts the compromised clients during FL training. This allows the adversary to mount stronger attacks. Note that model poisoning are naturally online attacks.   \\ 
&  & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-online.pdf}} \\ \hline
% \hline





% \hline



% \multirow{4}{2cm}{FL setting} & \multirow{2}{1.5cm}{Cross-silo} & All the clients send their updates to the server in each FL round. This allows adversary to continuously corrupt the global model and have more impactful attacks. \\
% &  & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-crosssilo.pdf}}\\ \cline{2-3}

% & \multirow{2}{1.5cm}{Cross-device} & Only a small fraction of the clients send their updates to the server in each FL round. Many FL rounds may have negligible number of malicious clients, and hence, making attacks more challenging. \\ 
% &  & \multicolumn{1}{c|}{\includegraphics[scale=.5]{figures/threat_table/fl_poisoning-crossdevice.pdf}} \\  \hline


% \multirow{2}{2cm}{Aggregation algorithm} & Simple average & The server uses simple average to aggregate client updates.\\
% & Robust aggregation & The server uses some robust aggregation, e.g., coordinate-wise Median, to aggregate client updates. \\ \hline

\end{tabular}
% \vspace{-6em}
\end{table*}





\section{Dimensions of the poisoning threat to FL}\label{poisoning_dimensions}

In this section, we discuss the four major dimensions of the poisoning threat that federated learning faces.
Specifically, they are: 1) adversary's goal, 2) adversary's knowledge of the global model, 3) adversary's manipulation capabilities, and 4) the mode of poisoning attacks.
In practice, each of the dimensions can take two possible values.
We define and compare the values of these dimensions in detail. Note that, a valid combination of values of various dimensions constitutes a specific threat model of poisoning attack on FL.

\begin{comment}
\red{
- we want to explain various dimensions in table
- we want to elaborate the practical threat models
}
\blue{
- we can merge adversary's capability and knowledge of global model
- sequece: goal, adversary's capability, attack model, FL setting, data distribution
- fl setting and data distribution are not really parts of threat model; how to incorporate?
}


- write all dimensions of threat model
- write all possible threat models combining the dimensions
- 
\end{comment}

\subsection{Adversary's goal}
\label{pd:goal}

The goal can be either \emph{untargeted} or \emph{targeted} poisoning: The untargeted poisoning forces the global model to misclassifies \emph{any} test input at the inference time. These attacks are more severe as they can completely cripple FL similar to the denial-of-service attacks. However, they are also less stealthy and more challenging to mount.

On the other hand, the targeted poisoning results in a global model that misclassifies the inputs with specific properties of the adversary's choice, while classifies all other inputs correctly. By definition, these attacks can target a subpopulation of clients, a single client, or even a sample. Therefore, targeted attacks are more stealthy and relatively easy to mount in practice.



\subsection{Adversary's capabilities}
\label{pd:capability}

\red{
divide cap in three things:
2 subsection under 3.2
- mp vs dp 
- offline vs online
sec 3.3: knowledge
- graybox: arch known. 

Online + DP makes little sense, bcs it's not possible to ship so much data in time, as it requires the knowledge of start of FL training, time of FL round, knowledge of FL round number, etc. Knowledge 
}

Based on the adversary's capability to \emph{manipulate} client devices, poisoning in FL can be either \emph{model poisoning} or \emph{data poisoning}. 
Note that, this is different from the adversary's capability to \emph{access} client devices, which we will discuss shortly.


In model poisoning, adversary directly manipulates the model update that the client sends to the server. While in data poisoning, the adversary only manipulates the training data on the client device. These contrasting assumptions present an interesting tradeoff between practicality (or feasibility) and efficacy (or impact) of poisoning in FL and below we discuss it in detail.


\paragraphb{\em Model poisoning.}
% 
Due to her ability to directly manipulate updates, the model poisoning adversary can craft arbitrarily malicious model updates and mount strong poisoning attacks on FL. 
However, due to advanced security firewalls and attestation protocols in modern operating systems, it is not trivial to access and manipulate model updates on client devices. 
More specifically, the adversary will have to break in to each of the client devices, successfully gain root access to the device (if the FL application does not run on rooted devices, the process further complicates), circumvent security firewalls and attestations, and modify FL training binaries. 
As the adversary cannot physically access client devices, model poisoning expects the \red{compromised clients} to have the aforementioned skills required to break in to a device. In practice, the adversary may find only a negligible number of such highly skilled clients in FL, which severely restricts the practical deployment of model poisoning attacks on FL~\cite{kozinski2017adversarial,bhagoji2019analyzing}. Specifically, in our experiments, we assume that adversary can directly corrupt the updates of up to 2\% client devices.


\paragraphb{\em Data poisoning.}
% 
On the other hand, data poisoning adversary in FL requires access to data on client devices, which in practice translates to just getting consent of the device owners. An example scenario to obtain such consent includes giving appropriate incentive to (e.g., bribing) the device owners participating in FL and installing a malicious application on their devices. Once the device owners allow the malicious application to access devices' data folders, adversary can easily download poisoning data on the devices as necessary. Hence, compromising clients for data poisoning on FL demands absolutely no skills from the device owners, which allows to deploy data poisoning in FL at a massive scales. Specifically, in our experiments, we assume that adversary can corrupt the training data of up to 10\% client devices.

However, data poisoning cannot craft arbitrarily malicious updates. Because, it manipulates the updates indirectly through poisoning the training data and it is not possible to craft \emph{valid} poisoning data for any malicious update. Figure~\ref{} demonstrates this for a simple logistic regression classifier. This limits the poisoning impact of malicious updates on FL and makes data poisoning significantly challenging.


\paragraphb{\em Model versus Data Poisoning.}
% 
As discussed above, the model poisoning adversary assumes complete control of the compromised client devices in order to circumvent security firewalls of their devices.
Hence, although in theory, model poisoning adversary can craft highly malicious updates for a given FL setting, the number of clients she can compromise is generally small, e.g., on order of up to 2\%~\cite{kairouz2019advances}. 
Figure~\ref{fig:mp_vs_dp} demonstrates the difference in capabilities of data and model poisoning adversaries.

Although it is possible to craft arbitrarily malicious updates using model poisoning attack, they  need not map to the valid data domain. 
\red{better visual example?}
% 
% \begin{comment}
For instance, in case the model parameters are zero, the gradients of those parameters will always be zero. In this example, for those specific parameters, model poisoning gradients can have any (nonzero) values, however, data poisoning gradients can only have zero values.
Furthermore, data samples generally have domain constraints, which makes the mapping even more challenging.
For instance, MNIST image classification task~\cite{lecun1998gradient} has $28\times 28$ gray-scale (8 bit) images, that is the input data domain consists of  $256^{784}$  possible images, however, the gradient domain is infinite ($\mathbb{R}^{d}$). This clearly shows the impossibility of mapping arbitrary gradients to data domain.
% \end{comment}


This makes data poisoning in FL significantly more challenging than model poisoning.
However, as the data poisoning adversary requires the compromised clients to simply inject poisoned data used to compute malicious gradients on their devices, the clients need not be skilled.
% 
Therefore, such adversary can compromise a larger number of clients in FL, e.g., up to 10\%~\cite{kairouz2019advances}.



\subsection{Adversary's knowledge of global model}
\label{pd:knowledge}

Adversary's knowledge of the global model in FL can be either \emph{Nobox} or \emph{Whitebox}. In the Nobox case, the adversary has no visibility in to the global model at all. This is the most challenging setting for the adversary as she will have to mount the attacks without any model or rely on some surrogate model.
But, this is also the most practical setting, as most FL applications' data, e.g., training code, binaries, model parameters, etc., are proprietary and protected by various security features of modern operating systems. 


In the Whitebox case, the adversary can access the global model parameters on compromised client devices. This is a very strong assumption on the adversary's knowledge, but it also allows her to craft more malicious updates via model or data poisoning. This setting is less relevant in practice, and therefore, we assume that the number of devices whose model parameters the adversary can access are very few, e.g., on order of 1-2\%~\cite{kairouz2019advances}.



\subsection{Attack mode}
\label{pd:mode}

The adversary can mount either \emph{online} or \emph{offline} poisoning attacks on FL.
In offline poisoning, the adversary corrupts the compromised client devices only onces, preferably at the beginning of FL training. 
For example, in label flip attacks~\cite{fang2020local}, the adversary flips the labels of benign data on compromised devices only once at the beginning of FL training.
Offline attacks are more feasible, and hence, more practical, as they do not require the adversary to access the client devices. 
However, these attacks are also less impactful, because, the effect of poisoning can quickly fade away in later FL rounds~\cite{bagdasaryan2018how}. 




On the other hand, in online poisoning, the adversary repeatedly corrupts the client devices.
For example, a model poisoning adversary manipulates the model updates in every FL round~\cite{fang2020local,baruch2019a,bhagoji2019analyzing,bagdasaryan2018how}. These attacks require the adversary to intrude the client devices repeatedly, which limits their applicability in practice.
However, these online attacks can be much more powerful than offline attacks,  as the adversary can maintain the attack impacts over the entire FL training.   



\begin{comment}
\subsection{FL setting}

There are two major types of FL settings: \emph{cross-silo} and \emph{cross-device} FL and use of the one or the other can affect the efficacy of poisoning attacks.
In cross-silo FL, the clients involved are generally large organizations, e.g., banks and hospitals, and the number of clients is generally smaller, e.g., 2-100~\cite{kairouz2019advances}. In each FL round, all of the clients receive the global model and share their updates with the server. This allows the adversary to poison the global model in each FL round, as the server selects all of the malicious clients. Hence, the poisoning attack can be more impactful.

On the other hand, in cross-device FL, the clients involved are individual who own a mobile device, e.g., Android cellphone, and the number of clients is very large, e.g., on order of $10^6$~\cite{kairouz2019advances}. In each FL round, the server randomly selects a small fraction of clients, shares the recent global model with them, and collects their updates. 
Due to the random subsampling, the server may select very few or even none of the malicious clients in many FL rounds. This limits the adversary's ability to continuously corrupt the global model and can reduce the impact of poisoning attacks on FL as Fang et al.~\cite{fang2020local} show.
\end{comment}

















% next, we can either define specific threat models in this section or directly in the section where attack methodology will be discussed.




==> method_dp.tex <==
% !TEX root = main.tex

\section{Our Data Poisoning Attack Methodology} \label{method}

% In our work, we focus on data poisoning attacks, which are more practical in nature, and therefore, easy-to-deploy on real world FL systems at massive scales. 
% Next, we consider the untargeted poisoning attacks, which severely hurt all of the FL clients in denial-of-service fashion.
% Finally, we consider the cross-device FL in our work, which is more prone to poisoning attacks than cross-silo setting. Because, the clients in cross-silo FL are large organizations, e.g., banks and hospitals, while the clients in cross-device FL are individual users who use mobile device, e.g., cellphones. As it is significantly more challenging to compromise a bank or a hospital compared to an individual user, cross-device FL is at a much higher risk of poisoning attacks.

% Below, we present the overview of our data poisoning attack framework, then specify AGR-specific conditions required to circumvent robust AGR algorithms, and finally present specific attacks under three data poisoning threat models.

% \begin{algorithm}
% \caption{General data poisoning algorithm}\label{alg:general_framework}
% \small{
% \begin{algorithmic}[1]
% \State \textbf{Input}: $\theta_t$, $\nabla_{\{i\in[m]\}}$, $f_\mathsf{agr}$ 
% % \State $D_p\leftarrow (\mathbb{R}^{n\times d}, Y^n)$
% % \Comment{Randomly initialize poisoning data}
% \For{$i\in\{1,2,...,T\}$}
% 	\State $D^i_p\leftarrow$ \texttt{COMPUTE\_POISON}$(D^{i-1}_p, \theta_t)$
% 	\State $b\leftarrow$ \texttt{CIRCUMVENTION\_CHECK}$(D^i_p, \nabla_{\{i\in[m]\}}, f_\mathsf{agr})$
%   	\If {$b\neq 1$}
%     	\State \textbf{return} $D^{i-1}_p$
%   	%\Else 
%   	\EndIf
% \EndFor
% \State \textbf{return} $D^T_p$
% % \State\textbf{Output} $\gamma_\mathsf{succ}$
% \end{algorithmic}
% }
% \end{algorithm}


% \subsection{Overview of our data poisoning attack}


% Our data poisoning attacks aim to compute a poisoning data $D_p$ such that when malicious clients compute their updates using $D_p$ and share them with the server, the resulting global model misclassifies any input to it. 
% 
Our attacks execute in two independent steps (we will shortly explain why we decouple these steps): In the first step, they compute poisoning data $D^g_p$. In the second step, they use Monte Carlo approach to sample the final poisoning data $D_p$ from $D^g_p$ such that $D_p$ circumvents the server's AGR algorithm and also corrupts the global model.
% 


% Our attacks execute in two independent steps: In the first step, we use \texttt{COMPUTE\_POISON} subroutine to compute poisoning data, $D^g_p$ and in the second step, we use \texttt{CIRCUMVENTION\_CHECK} subroutine to tune $D^g_p$ and obtain final poisoning data $D_p$ such that the corresponding model updates can circumvent robustness criterion of the server's AGR, if any.


\subsection{Step-1: Compute poisoning data}
% \red{formalize the objective, argue why it is hard to solve directly, give relation between the objective and amount of label flipped data, state and reason about how different types of label flips lead to different objective values, simplify the objective}


This step computes poisoning data, $D^g_p$, such that the corresponding model updates computed using fedAVG algorithm corrupt the global model in an untargeted fashion.
Therefore, our objective is to compute $D_p$ such that when global model, $\theta^g$, is updated using $D_p$ and a learning algorithm $A$, e.g., stochastic gradient descent, it will have high loss on some benign test data, $D_b$. This objective is formalized below:
% 
\begin{align}\label{eq:objective}
&\underset{D_p\subset \mathbb{D}}{\text{argmax}}\ \ L(D_b;\theta')\quad\quad \text{where }\theta' \leftarrow A(D_p, \theta^g)
\end{align}

In fedAVG, the learning algorithm $A$ updates $\theta$ multiple times using minibatches of $D_p$. To solve this optimization in~\eqref{eq:objective}, the attacker should use the back-gradient optimization based approach~\cite{munoz2017towards}.
However, back-gradient optimizations are extremely slow: \cite{fang2020local} reports run time of 10 days on a single GPU to compute 240 poisoning samples for logistic regression classifier trained on MNIST task. This makes it impossible to use in federated learning, where a typical FL round lasts for 15-20 minutes~\cite{kairouz2019advances} and which uses large neural networks such as VGG and ResNet.
Furthermore, and more disappointingly, these attacks have no noticeable impacts on federated learning~\cite{fang2020local} or centralized machine learning~\cite{munoz2017towards}. Because, even the back-gradient propagation based solutions to~\eqref{eq:objective} are not optimal solutions due to the non-convexity of~\eqref{eq:objective}.


Instead we propose to use benign data on malicious devices and flip their labels in a particular fashion to solve~\eqref{eq:objective}.
The choice of label flipped data may not be the optimal with respect to the objective in~\eqref{eq:objective}.
But, we exploit the very salient feature of FL that the server has no visibility in to the data on client device to maximally satisfy~\eqref{eq:objective}. 
More specifically, we observe in Figure~\ref{fig:obj_explnation} (left-most) that increasing the size of $D^g_p$, increases the loss $L(D_b;\theta')$ in~\eqref{eq:objective}, and therefore, finds a better solution to~\eqref{eq:objective}.
% Finally, we will show that the efficacy of these attacks depends significantly on how does the adversary deploy the poisoning data across the compromised devices.


\paragraphb{\em Label flipping strategies.}
We propose two label flipping strategies: \emph{static} label flipping (\texttt{SLF}) and \emph{dynamic} label flipping (\texttt{DLF}).
In \texttt{SLF}, the adversary flips the label of a given sample in a fixed manner, i.e., for a sample $(\mathbf{x},y)$, she changes the true label $y$ to $C-1-y$, where $C$ is the total number of classes.
On the other hand, in \texttt{DLF}, given a model $\theta$, the adversary flips the true label $y$ to the least probable label with respect to $\theta$, i.e., to ${argmin}\ \theta(\mathbf{x})$.


\paragraphb{\em Computing flipped labels for online attacks.}
Static label flipping is straight forward as described before.
However, for dynamic label flipping, adversary requires a model, but note that she cannot access the actual global model. 
Hence, we first describe a way to obtain such model.


Recall that, the adversary has access to the benign data on compromised devices.
We propose to use this benign data and train multiple \emph{shadow models} using fedAVG algorithm.
For instance, if the adversary compromises 100 out of 1000 total FL clients, she uses fedAVG algorithm for multiple rounds and trains multiple shadow models (one per round) using the 100 compromised clients.


Finally, we propose to use the shadow model from the $i^{th}$ orchestrated FL round as the replacement for the global model from the $i^{th}$ actual FL round, and compute the \texttt{DLF} poisoning data.



\paragraphb{\em Computing flipped labels for offline attacks.}
% Computing \texttt{SLF} poisoning data for offline attacks is straightforward and is similar to the online case.
Static label flipping is straight forward as described before.
However, unlike in online attacks, in offline attacks, the adversary corrupts compromised clients' local data just once.
Hence, to compute \texttt{DLF} poisoning data for offline attacks, adversary should select a model from the multiple shadow models she computes by orchestrating FL.
We propose to use the best model obtained during the orchestrated FL training, but in Section~\ref{results}, we also explore the effect of using different models on the attack efficacy.



\paragraphb{\em Impact of different label flipping strategies.}
Figure~\ref{fig:obj_explnation} (left) shows how increasing the size of poisoning data used to update the global model increases the loss on some validation data, i.e., shows how increasing $D_p$ increases loss $L(D_b;\theta')$ in~\eqref{eq:objective}. The norm of the corresponding malicious updates also increases with $|D_p|$, which as we show suffices to jeopardize averaging based AGRs that are the most widely adopted in practice.
\texttt{DLF} increases $L(D_b;\theta')$  significantly more than \texttt{SLF}, because \texttt{DLF} is more tailored to the model $\theta$ in~\eqref{eq:objective}.

\subsection{Step-2: Tune poisoning data}



% The second step of our attack finds a subset of the poisoning data, $D^g_p$, from the first step that circumvents the server's AGR.
In the second step of our attack, we design an AGR-specific attack optimization problem that finds the optimal subset of $D^g_p$ such that the corresponding malicious updates circumvent the AGR's robustness constraints.
% 


For instance, Multi-krum AGR uses Krum AGR to filter a specific number of its input model updates.
The larger the subset of $D^g_p$, the corresponding update will be more malicious. But, it will also be farther away from the benign updates and Krum will filter it.
Hence, our attack optimization aims to find the largest subset of $D^g_p$ such that Krum AGR will select all of the corresponding malicious update.



In our work we study four AGRs which are representatives of four different types of aggregation algorithms: (1) \emph{Weighted average} is the most widely adopted AGR, (2) \emph{Multi-krum} represents geometric median based AGRs, (3) \emph{Trimmed-mean} represents coordinate-wise filtering based AGRs, and (4) \emph{RSA} represents updates' signs based AGRs.
% 


Below, we first describe a general attack optimization framework and an algorithm to solve the optimization for any given AGR. Then we detail the specific optimization problems for each of the aforementioned AGRs.


\subsubsection{General attack optimization problem}


For a give AGR algorithm $f_\mathsf{agr}$, our attack optimization finds $D_p\subset D^g_p$ such that the corresponding model updates deviate $\theta^g$ maximally towards the inverse of the direction in which $\theta^g$ would change in the absence of any attacks.
% 
We formalize this in~\eqref{eq:gen_opt}.
% 
\begin{align}\label{eq:gen_opt}
&\underset{D_p\subset D^g_p}{\text{argmax}}\quad s^T(\widetilde{\nabla} - \widetilde{\nabla}^m) \\
\text{s.t.}\quad s=&\text{sign}(\widetilde{\nabla}),\quad \widetilde{\nabla} = f_\mathsf{agr}(\nabla_{i\in\{[1,n]\}})\nonumber \\
\widetilde{\nabla}^m = &f_\mathsf{agr}(\nabla^m_{i\in\{[1,m]\}}, \nabla_{i\in\{[m+1,n]\}})\nonumber
\end{align}
% 
where $s^T$ is the transposed vector of signs of the average of model updates, when there are no attacks, i.e., $s=\text{sign}(\widetilde{\nabla})$.
We assume that there are $m$ malicious clients out of total $n$ clients, and
$\nabla_i$ and $\nabla^m_i$ are the updates corresponding to the benign and malicious clients, respectively.


Note that our optimization framework is derived from the bi-level optimizations used in the long ling of research on poisoning attacks in central~\cite{biggio2014poisoning,munoz2017towards,biggio2012poisoning} and federated learning~\cite{fang2020local}. 
% 
Solving this optimization under model poisoning~\cite{fang2020local} case is straightforward, but is significantly challenging for the data poisoning case, in part due to the fundamental difficulty of generating poisoning data that imitates the model poisoning updates.


\begin{algorithm}
\caption{Step-2: Tune poisoning data in $i^{th}$ FL round}\label{alg:mc_solution}
% \small
{
\begin{algorithmic}[1]
\State \textbf{Input}: $\hat{\theta}_i$, $D^g_p$, $f_\mathsf{agr}$, $\nabla_{\{i\in[n-m]\}}$
\State $\widetilde{\nabla}\leftarrow f_\mathsf{agr}(\nabla_{\{i\in[n-m]\}})$ \Comment {Compute a benign aggregate}
\State 
\State \hspace{6em}\textbf{\em Compute optimal $D_p$ size}
% \State 
\State $|D_p|^*\leftarrow 0$
\Comment {Initialize best $|D_p|$ to 0}

\For{$D\in[1,|D^g_p|]$}
	\State $D_p\sim D^g_p$ \Comment {Subsample $D_p$ of size $D$}
	\State $\nabla^m\leftarrow A(D_p,\hat{\theta}_i)$ \Comment {Compute malicious update}
	% \State $\widetilde{\nabla}^m\leftarrow f_\mathsf{agr}(\nabla^m_{i\in[m]}\cup \nabla_{\{i\in[n-m]\}})$ \Comment {Compute poisoned aggregate}
	% \State $\texttt{dev}\leftarrow \Vert\widetilde{\nabla} - \widetilde{\nabla}^m\Vert_2$ \Comment {Compute deviation}
	\State $b\leftarrow \texttt{CHECK\_CRITERION}(\nabla^m,\nabla_{\{i\in[n-m]\}},f_\mathsf{agr})$
	\If{$b=1$} \Comment {If $D$ satisfies the criterion}
		% \State $\texttt{dev}^*\leftarrow \texttt{dev}$
		% \Comment {Update best deviation to $\texttt{dev}$}
		\State $|D_p|^*\leftarrow D$
		\Comment {Update best $D_p$ size to $D$}
	\EndIf
	\State $D\leftarrow D+\delta$
	\Comment {Repeat with larger $D_p$ size}
\EndFor

\State 
\State \hspace{2em}\textbf{\em {Obtain $D_p$ that maximizes inverse deviation}}
% \State

\State ${s}^*\leftarrow -\text{sign}(\widetilde{\nabla})$
\Comment {Compute the target inverse direction}
\State ${sd}^*\leftarrow \text{len}(s^*)$ \Comment{Initialize sign-diff variable}

\State $D^*_p\leftarrow \emptyset$ \Comment{Initialize the best $D_p$ variable}

\For{$t\in[1,T]$}
	\State $D_p\sim D^g_p$ \Comment {Sample $D_p$ of size $|D_p|^*$}
	\State $\nabla^m\leftarrow A(D_p,\hat{\theta}_i)$
	\State $sd\leftarrow \Vert \text{sign}(\nabla^m)-{s}^* \Vert_1$
	\Comment{Compute $L_1$-distance}
	\If {$sd < {sd}^*$}
		\State $D^*_p\leftarrow D_p$, ${sd}^* \leftarrow sd$
		\Comment {Update the variables}
	\EndIf
\EndFor

\State\textbf{Output} $D^*_p$

\end{algorithmic}
}
\end{algorithm}




\begin{algorithm}
\caption{Circumvention criterion for \texttt{TrMean}}\label{alg:trmean}
% \small
{
\begin{algorithmic}[1]
\State \textbf{Input}: $\widetilde{\nabla}$, $\nabla^m$, $\nabla_{\{i\in[n-m]\}}$, $\texttt{dist}^*\leftarrow\text{max}(\Vert\widetilde{\nabla}-\widetilde{\nabla}^m\Vert)$ so far
\State $\widetilde{\nabla}^m\leftarrow f_\mathsf{TrMean}(\nabla^m_{\{i\in[m]\}}\cup \nabla_{\{i\in[n-m]\}})$ \Comment {Poisoned aggregate}
\State \textbf{output} $(\Vert\widetilde{\nabla}-\widetilde{\nabla}^m\Vert > \texttt{dist}^*)$
\end{algorithmic}
}
\end{algorithm}


\begin{algorithm}
\caption{Circumvention criterion for \texttt{RSA}}\label{alg:rsa}
% \small
{
\begin{algorithmic}[1]
\State \textbf{Input}: $\widetilde{\nabla}$, $\nabla^m$, $s^*\leftarrow\widetilde{\nabla}$, $\texttt{dist}^*\leftarrow\text{min}(\Vert\text{sign}(\widetilde{\nabla}^m)-s^*\Vert_1)$ so far
\State \textbf{output} $(\Vert\text{sign}(\widetilde{\nabla}^m)-s^*\Vert_1 < \texttt{dist}^*)$
\end{algorithmic}
}
\end{algorithm}


\begin{algorithm}
\caption{Circumvention criterion for \texttt{MKrum}}\label{alg:mkrum}
% \small
{
\begin{algorithmic}[1]
\State \textbf{Input}: $\nabla^m$, $\nabla_{\{i\in[n-m]\}}$, $|D_p|^*\leftarrow$ largest $|D_p|$ s.t. $f_\mathsf{mkrum}$ selects all of corresponding $\nabla^m$
\State $\mathcal{S}\leftarrow f_\mathsf{mkrum}(\nabla^m_{i\in[m]}\cup \nabla_{\{i\in[n-m]\}})$ \Comment{Compute selection set}
\State \textbf{output} $m\leq|\{\nabla^m\in\mathcal{S}\}|$
% \State \textbf{output} $(\Vert\text{sign}(\widetilde{\nabla}^m)-s^*\Vert_1 < \texttt{dist}^*)$
\end{algorithmic}
}
\end{algorithm}



\paragraphb{\em Approach to solving the attack optimization.}
We propose to use Monte Carlo (MC) optimization approach, where a random sample is repeatedly drawn from a pre-defined solution domain and the sample that maximizes the objective is used as the final solution.
These methods are shown to effectively solve optimizations in machine learning~\cite{}, and as we show are effective in solving our attack optimization as well.

% To use the MC approach, we should first decide the size of $D_p$ to sample from $D^g_p$. Because, as we show in Figure~\ref{}, sampling $D_p$ of random 
First, we separate the two parts of the maximization in~\eqref{eq:objective}: First maximizes the deviation $\Vert\widetilde{\nabla}-\widetilde{\nabla}^m\Vert$, i.e., maximally circumvents the given robust AGR. While second maximizes alignment of the deviation with the inverse of a benign direction, i.e., aligns with $-s$. We propose to separately solve the two parts of the optimization.
% 

To maximize the deviation for a given AGR, we observe that, a specific size of $D_p$ maximally circumvents the robustness criterion of the AGR. Hence, we design a circumvention criterion check based on the knowledge of the AGR.
%
For instance, in Multi-krum, the higher the size of $D_p$, $|D_p|$, the higher the deviation of the corresponding malicious updates from the benign updates, which lowers their chances of Multi-krum selecting them. Hence, we find a suitable $|D_p|$ such that Multi-krum selects all of the corresponding malicious updates.


% 
Once, we have $|D_p|$, we invoke MC approach and repeatedly sample $D_p\subset D^g_p$ of size $|D_p|$, and use the $D_p$ whose corresponding update maximally aligns with $-s$.
We note that, similar to~\cite{fang2020local}, we also tried to mount attacks that only maximize the deviation $\Vert\widetilde{\nabla}-\widetilde{\nabla}^m\Vert$ and observe that they have lower attack impacts than maximizing the inverse deviation.
% 

It is worth emphasizing that we explored an generator networks based alternating maximization approach: We generated $D_p$ of fix size using generator network~\cite{yang2017generative} and alternated between maximizing the deviation and maximizing the alignment with $-s$. But, we observe that such attacks do not outperform the label flipping based attacks we present and their success depends on our observation about the relation between $|D_p|$ and maximizing the deviation. Furthermore, such generators based attacks are significantly challenging for categorical and text datasets.
% plays the prime role in attacks' success. Furthermore, such generator based attacks  and are also computationally demanding. 
% On the other hand, our assumption of the strong correlation between the size of $D_p$ and maximizing the deviation for a given AGR leads to strong data poisoning attacks on FL. 
% Hence, we leave further investigation in to solving~\eqref{eq:gen_opt} to future work.


\paragraphb{\em Overview of our attack algorithm.}
Below we explain our attack algorithm for $i^{th}$ FL round given in Algorithm~\ref{alg:mc_solution}.
We first describe the algorithm for online attacks, and then explain how to use it for offline attacks.

We first compute the optimal $|D_p|$, i.e., $|D_p|^*$, by performing a grid-search over a large spectrum of possible sizes of $D_p$, denoted by $D$.
For each possible $D$, we sample $D_p$ from available label flipped data and compute the corresponding malicious update (Lines 7-8). 
We compute a specific number of benign updates, $\nabla_{\{i\in[n-m]\}}$, using the available benign data and shadow model (Line 1). Here $n$ is the number of clients selected in each FL round and $m$ is fixed based on the \% of compromised clients in the system.
Next, we check whether a set of $m$ replicas of the malicious update can satisfy an AGR-tailored circumvention criterion (Line 9). If it does, we update $|D_p|^*$ to current $D$ and repeat the process with larger $D$ (Line 10-12); the step $\delta$ used to increase $D$ is a hyperparameter (Line 13).
% Finally, we use as the optimal $|D_p|^*$, the maximum of $|D_p|$'s that circumvent the circumvention criterion.


The second step of our attack algorithm uses MC approach to find the $D_p\subset D^g_p$ of size $|D_p|^*$ that maximizes the inverse deviation and is AGR-agnostic.
Specifically, we sample $D_p$ and compute corresponding malicious update (Line 21-22), and compute the $L_1$-norm distance between the target inverse direction $s^*$ (Line 17)  and sign of the malicious update (Line 23).
The lower the $L_1$-norm distance, the more malicious the $D_p$. We can obtain more malicious $D_p$ by repeating the process (Line 21-25) more number of times.


In case of offline attacks, adversary can corrupt compromised devices' data only once. Hence, we propose to use the best available shadow model to compute the best $D_p$ using Algorithm~\ref{alg:mc_solution}.
As changing the shadow model we use in Algorithm~\ref{alg:mc_solution} changes $|D_p|$, we evaluate the impact of varying $|D_p|$ on offline attacks' efficacy in Section~\ref{exp:dp_compare}.



\subsubsection{AGR-specific circumvention criterion}
In this section, we describe each of the AGR algorithms we study in this work and provide circumvention criteria for them.

\paragraphb{\em Weighted average.}
In each FL round, weighted average (\texttt{wtAVG}) assigns weights to an input update proportional to the size of data used to compute the update, and then computes a weighted average of all of the input updates.
% 

Although \texttt{wtAVG} provides no theoretical robustness, it is important to study for two reasons: 1) it is the only AGR used in practical FL applications~\cite{kairouz2019advances,mcmahan2017communication}, 2) previous data poisoning attacks are completely ineffective against \texttt{wtAVG}, which can give a false sense of security.
% 
Figure~\ref{fig:obj_explnation} shows that increasing $|D_p|$, increases the poisoning impact of the corresponding malicious updates as well as arbitrarily increases their norm.
Therefore,
 % and because \texttt{wtAVG} does not impose any robustness constraints on its inputs
we use all of $D^g_p$ on each of the compromised client devices. 
If necessary, we generate more malicious data by arbitrarily perturbing existing $D^g_p$ in order to increase the weight of malicious updates.
% 
Using all of $D^g_p$ results in highly malicious updates with significantly higher weights than the benign clients.


\paragraphb{\em Trimmed-mean.}
In each FL round, $\beta$-Trimmed-mean (\texttt{Trmean}) AGR~\cite{yin2018byzantine} filters $\beta$ fraction of maximum and minimum values along each of the dimensions of model updates collected at the server.
Then it averages the remaining values along each of the dimensions.
% 

For a given set of benign updates, our circumvention criterion for \texttt{Trmean} (Algorithm~\ref{alg:trmean}) checks which size of $D_p$ maximizes the deviation $\Vert\widetilde{\nabla}-\widetilde{\nabla}^m\Vert$ between the benign and malicious aggregates computed using \texttt{Trmean}.
In Figure~\ref{fig:obj_explnation}, we observe that increasing the size of $D_p$ increases the deviation $\Vert\widetilde{\nabla}-\widetilde{\nabla}^m\Vert$. Therefore, in our experiments we keep $|D_p|$ close to $|D^g_p|$.
% 
This maximization combined with maximizing the inverse deviation in the second step of our attack imitates the attack by Fang et al.~\cite{fang2020local} on \texttt{Trmean}.



\paragraphb{\em RSA.}
RSA aggregation algorithm requires an FL client to train her model update using $L_p$-norm regularization, i.e., ensure that the resulting and original models, $A(D_i, \theta^g)$ and $\theta^g$, are close in some $L_p$-norm space (we use $L_1$ norm as suggested in the paper).
The client then computes the sign of the difference $A(D_i, \theta^g) - \theta^g$ as her final update. Finally, the server averages all of the received updates.


Note that, as the model updates in RSA are sign vectors, our circumvention criterion for \texttt{RSA} (Algorithm~\ref{alg:rsa}) checks which size of $D_p$ can maximize the inverse deviation, and uses this $D_p$ size in the second step of our attack.
In Figure~\ref{fig:obj_explnation}, we observe that increasing the size of $D_p$ beyond a particular threshold size optimizes our attack objective, i.e., reduces $\Vert\text{sign}(\widetilde{\nabla}^m)-s^*\Vert_1$. Therefore, in our experiments we keep $|D_p|$ close to $|D^g_p|$.



\paragraphb{\em Multi-krum.}
Multi-Krum AGR~\cite{blanchard2017machine} (\texttt{Mkrum}) selects an update using Krum AGR~\cite{blanchard2017machine} from a remaining-set (initialized to the set of all the received updates), adds it to a selection-set (initialized to an empty set), and removes it from the remaining-set. This way, Multi-krum selects $c$ updates such that $n-c > 2m+2$. Finally, Multi-krum averages the updates in the selection-set. 
We omit Krum from our work due to its unacceptably low performance in non-iid FL settings, and instead evaluate Multi-krum which provides performance equivalent to weighted average and robustness equivalent to Krum.



Our \texttt{Mkrum} circumvention criterion (Algorithm~\ref{alg:mkrum}) checks which $D_p$ size gives malicious updates such that \texttt{Mkrum} selects all of them.
Ensuring that \texttt{Mkrum} selects all malicious updates maximizes their malicious updates and minimizes the good impact of benign updates.
We note in Figure~\ref{fig:obj_explnation} that there is an optimal $|D_p|$ close to the average of benign clients' data that maximizes the number of malicious updates \texttt{Mkrum} selects.
Hence, in  our experiments, we search for such optimal $D_p$ in $[1, 3\cdot\widetilde{D}^b]$, where $\widetilde{D}^b$ is the average  of benign clients' data.
We keep all of the malicious updates the same to increase their chances of getting selected.




==> method_mp.tex <==
% !TEX root = main.tex

\section{Our Model Poisoning Attack Methodology} \label{method}


==> pgfplotstableset.tex <==
\pgfplotstableset{
    /color cells/min/.initial=0,
    /color cells/max/.initial=1000,
    /color cells/textcolor/.initial=,
    %
    % Usage: 'color cells={min=<value which is mapped to lowest color>, 
    %   max = <value which is mapped to largest>}
    color cells/.code={%
        \pgfqkeys{/color cells}{#1}%
        \pgfkeysalso{%
            postproc cell content/.code={%
                %
                \begingroup
                %
                % acquire the value before any number printer changed
                % it:
                \pgfkeysgetvalue{/pgfplots/table/@preprocessed cell content}\value
                \ifx\value\empty
                    \endgroup
                \else
                \pgfmathfloatparsenumber{\value}%
                \pgfmathfloattofixed{\pgfmathresult}%
                \let\value=\pgfmathresult
                %
                % map that value:
                \pgfplotscolormapaccess
                    [\pgfkeysvalueof{/color cells/min}:\pgfkeysvalueof{/color cells/max}]
                    {\value}
                    {\pgfkeysvalueof{/pgfplots/colormap name}}%
                % now, \pgfmathresult contains {<R>,<G>,<B>}
                % 
                % acquire the value AFTER any preprocessor or
                % typesetter (like number printer) worked on it:
                \pgfkeysgetvalue{/pgfplots/table/@cell content}\typesetvalue
                \pgfkeysgetvalue{/color cells/textcolor}\textcolorvalue
                %
                % tex-expansion control
                % see https://tex.stackexchange.com/questions/12668/where-do-i-start-latex-programming/27589#27589
                \toks0=\expandafter{\typesetvalue}%
                \xdef\temp{%
                    \noexpand\pgfkeysalso{%
                        @cell content={%
                            \noexpand\cellcolor[rgb]{\pgfmathresult}%
                            \noexpand\definecolor{mapped color}{rgb}{\pgfmathresult}%
                            \ifx\textcolorvalue\empty
                            \else
                                \noexpand\color{\textcolorvalue}%
                            \fi
                            \the\toks0 %
                        }%
                    }%
                }%
                \endgroup
                \temp
                \fi
            }%
        }%
    }
}

==> practical_threat_models.tex <==
% !TEX root = main.tex

\section{Practical Threat Models in FL}

In our work, we consider a poisoning adversary whose goal is to mount the more challenging, but more severe, \emph{untargeted} poisoning attacks on FL. Given the poisoning adversary's goal, we can obtain eight possible threat models in FL by combining the rest of the three dimensions given in Table~\ref{table:poisoning_dimensions}. All of these combinations are given in Table~\ref{tab:threat_combinations}.
% 
However, not all of these combinations constitute valid threat models.   Below, we elaborate the valid threat models in FL and justify why the rest of combinations do not form valid threat models.

\begin{table}
\caption{Eight possible threat models for untargeted poisoning attacks on FL obtained by combining three dimensions from Table~\ref{table:poisoning_dimensions}: adversary's capability, adversary's knowledge, and attack mode.} \label{tab:threat_combinations}
\vspace{-.5em}
\centering
\begin{tabular} {|c|c|c|c|} %{@{} l*{5}{S} @{}}
  % \toprule
  \hline
  & Capability & Knowledge & Mode \\ 
  & $\mathcal{C}\in\{\texttt{mp},\texttt{dp}\}$ & $\mathcal{K}\in\{\texttt{nb},\texttt{wb}\}$ & $\mathcal{M}\in\{\texttt{off},\texttt{on}\}$ \\ \hline
  T1 & \texttt{mp} & \texttt{nb} & \texttt{off} \\ \hline
  T2 & \texttt{mp} & \texttt{nb} & \texttt{on} \\ \hline
  T3 & \texttt{mp} & \texttt{wb} & \texttt{off} \\ \hline
  T4 & \texttt{mp} & \texttt{wb} & \texttt{on} \\ \hline
  T5 & \texttt{dp} & \texttt{nb} & \texttt{off} \\ \hline
  T6 & \texttt{dp} & \texttt{nb} & \texttt{on} \\ \hline
  T7 & \texttt{dp} & \texttt{wb} & \texttt{off} \\ \hline
  T8 & \texttt{dp} & \texttt{wb} & \texttt{on} \\ \hline
 
\end{tabular}

\end{table}


\subsection{Details of valid threat models}
% Give specific capability, knowledge, mode, and then give scenarios

\paragraphb{\em Nobox offline data poisoning (T5).}
% 
This is the threat model T5 in Table~\ref{tab:threat_combinations} and  assumes an adversary who corrupts the data on compromised client devices, i.e., mounts a data poisoning (\texttt{dp}) attack, only once at the beginning of FL training (\texttt{off}) and has no knowledge of the global model (\texttt{nb}).
% 
We argue that this is the most practical threat model in FL because: First, the adversary does not perform the cumbersome task of breaking in to any devices which allows her to compromise more clients as argued in Section~\ref{pd:capability}. Second, the adversary corrupts the compromised clients' data only once, which further reduces the attack complexity.
% 
Such adversary requires basic knowledge of ML and some benign data (e.g., benign data on the compromised client devices) from the same distribution as the data of benign FL clients.
Note that, due to the weak assumptions on adversarial capabilities, such adversary can be any entity, e.g., an individual attacker or even a small organization who can bribe some of the FL clients.



\paragraphb{\em Nobox online data poisoning (T6).}
% 
This is the threat model T6 in Table~\ref{tab:threat_combinations} and  differs from T5 above only in terms of attack mode ($\mathcal{M}$). 
T6, allows its adversary to mount online attack (\texttt{on}), i.e., repeatedly corrupt the data on compromised client devices, while in T5 allows offline attack (\texttt{off}).
% 
T6 threat model requires the adversary to synchronize the corruption of data of compromised clients with the FL round. For instance, if round-$i$ takes 10 minutes, the adversary should corrupt the data precisely at the beginning of round-$i$ and ensure it is processed in 10 minutes. This is not trivial as the timing of an FL round might be variable and not a public knowledge. 
% 
In addition to the capabilities of T5 adversary, T6 adversary should also know the FL round timings and ensure that the poisoned data on compromised devices is processed in time. Therefore, T6 is relatively less practical than T5.




\paragraphb{\em Whitebox online model poisoning (T4).}
This is the strongest threat model in FL. It allows its adversary to directly access the global model (\texttt{wb}) and manipulate the model updates (\texttt{mp}) on compromised devices in every round of FL training (\texttt{on}).
% 
T4 threat model requires a very strong adversary who can break in to each of the compromised client devices, which is an impractically nontrivial task as argued in Section~\ref{pd:capability}.
Such adversary and also the client devices that she compromised should have advanced knowledge of security protocols of modern operating systems, e.g., Android, along with the knowledge of T6 detailed above. Due to such strong assumptions on adversary's and compromised clients' capabilities, T4 is an impractical threat to FL, but unfortunately the only one that previous literature considers~\cite{fang2020local,bagdasaryan2018how,baruch2019a,bhagoji2019analyzing}.





\subsection{Justifying invalidity of threat models}

We now justify the invalidity of the rest of threat models from Table~\ref{tab:threat_combinations}.
Model poisoning (\texttt{mp}) implicitly assumes whitebox access (\texttt{wb}) to the compromised devices, hence T1 and T2 are not valid threat models. Similarly, data poisoning (\texttt{mp}) implies that the adversary cannot access the global models on compromised devices (\texttt{nb}), hence T7 amd T8 are valid threat models. Finally, T3 threat model assumes an adversary with whitebox access to client devices who corrupts the model updates only once during FL training. Although valid, it is imprudent to perform the cumbersome task of breaking in to all the compromised devices to corrupt the model updates only once, hence, we believe T3 is also not a practical threat model.










